A POV-based Highway Vehicle Trajectory Dataset and Prediction Architecture

Vehicle Trajectory datasets that provide multiple point-of-views (POVs) can be valuable for various traffic safety and management applications. Despite the abundance of trajectory datasets, few offer a comprehensive and diverse range of driving scenes, capturing multiple viewpoints of various highway layouts, merging lanes, and configurations. This limits their ability to capture the nuanced interactions between drivers, vehicles, and the roadway infrastructure. We introduce the \emph{Carolinas Highway Dataset (CHD\footnote{\emph{CHD} available at: \url{https://github.com/TeCSAR-UNCC/Carolinas\_Dataset}})}, a vehicle trajectory, detection, and tracking dataset. \emph{CHD} is a collection of 1.6 million frames captured in highway-based videos from eye-level and high-angle POVs at eight locations across Carolinas with 338,000 vehicle trajectories. The locations, timing of recordings, and camera angles were carefully selected to capture various road geometries, traffic patterns, lighting conditions, and driving behaviors. We also present \emph{PishguVe}\footnote{\emph{PishguVe} code available at: \url{https://github.com/TeCSAR-UNCC/PishguVe}}, a novel vehicle trajectory prediction architecture that uses attention-based graph isomorphism and convolutional neural networks. The results demonstrate that \emph{PishguVe} outperforms existing algorithms to become the new state-of-the-art (SotA) in bird's-eye, eye-level, and high-angle POV trajectory datasets. Specifically, it achieves a 12.50\% and 10.20\% improvement in ADE and FDE, respectively, over the current SotA on NGSIM dataset. Compared to best-performing models on CHD, \emph{PishguVe} achieves lower ADE and FDE on eye-level data by 14.58\% and 27.38\%, respectively, and improves ADE and FDE on high-angle data by 8.3\% and 6.9\%, respectively.

==> Tex/motivation.tex <==
\section{Motivation: POV-based datasets and path prediction architectures}

% Previous section highlights the contemporary vehicle trajectory datasets and path prediction architectures. One common theme across most of the published work is that they do not have any component of POV-based safety applications. They either concentrate on birds-eye or dash-cam view for developing the trajectory datasets and prediction models for variety of applications. These approaches are very useful for most applications related to autonomous driving and post traffic analysis. However, they may not be as helpful for road-side safety applications and surveillance applications as camera angle may be very different and not many datasets are available foe these approaches.

The preceding section provided an overview of contemporary vehicle trajectory datasets and path prediction architectures. A common limitation among the published works is the lack of focus on POV-based safety applications. The majority of studies have focused on developing trajectory datasets and prediction models from either a bird's-eye view or a dashcam perspective, which are applicable to a variety of autonomous driving and post-traffic analysis applications. While these approaches have proven to be useful, they may not be adequate for road-side safety and surveillance applications. This is due to the fact that the camera angle may differ significantly, and the availability of datasets specifically designed for these types of applications is limited.


% Point-of-view (POV) datasets are critical for road-side safety, worker protection, and surveillance applications as they provide a comprehensive and detailed view of the environment from the perspective of a moving vehicles or workers. In road-side safety applications, POV datasets can be used to monitor traffic conditions, detect and track vehicles, predict and prevent accidents, and enhance road-side assistance. The data captured from POV cameras can provide valuable information about the road environment, including the position and speed of vehicles, the location and type of road obstacles, and weather conditions, which can be used to improve road safety.
POV based datasets are crucial for road-side safety, worker protection, and surveillance applications as they provide a more comprehensive and detailed view of the environment and the movements of objects within it. These datasets offer a unique perspective that is not available through traditional birds-eye view or dashcam based datasets. In road-side safety applications, POV based datasets can be used to monitor traffic conditions, predict traffic flow patterns, detect and track vehicles, and predict their movements and trajectories. This information can then be used to enhance road-side assistance, predict and prevent accidents, and provide real-time information about traffic conditions and road hazards.

In worker protection and surveillance applications, POV datasets are essential for monitoring the working conditions of employees and ensuring their safety. The data captured from POV cameras can be used to detect and alert on potential hazards, monitor compliance with safety procedures, and assess worker performance. POV datasets provide a rich source of information that can be used to train machine learning models and develop advanced computer vision algorithms. These algorithms can be used to analyze and interpret the data in real-time, providing insights into the environment and enabling the development of more effective safety, protection, and surveillance systems.

% Similarly, in worker protection and surveillance applications, POV based datasets can be used to monitor working conditions, ensure worker safety, assess worker performance and compliance with safety procedures, and improve worker efficiency by predicting and planning worker movements and tasks.

POV based trajectory prediction models are important for these applications as they use POV based datasets to train machine learning algorithms and develop more effective safety, protection, and surveillance systems. By predicting movements and trajectories in real-time, these models provide a deeper understanding of the environment and enable more proactive and effective responses to potential hazards and threats.





==> Tex/preliminaries.tex <==
\section{Priliminaries}

\subsection{POVs in vehicle trajectory prediction}
POV stands for "point of view" and refers to the camera angle or perspective from which the scene is captured. In deep learning trajectory prediction, different POV's can be used to capture the movement of vehicles or other objects in a scene. Some common POV's used in deep learning trajectory prediction are:

\begin{itemize}
  \item \textbf{Birds-eye view}: This is a top-down view of the scene, where the camera is placed directly above the area of interest. Birds-eye view can capture the movement of vehicles or pedestrians in a wider area and is commonly used in traffic analysis.
  \item \textbf{Dash cam view}: This is a front-facing view from a camera mounted on the dashboard of a car. The dash cam view captures the perspective of a driver, providing a more naturalistic view of the scene. Dash cam view is often used to predict the movement of other vehicles in a driving environment.
  \item \textbf{Eye-level view}:  This is a view captured from the height of an observer's eyes, providing a more realistic and intuitive view of the scene. Eye-level view is commonly used for pedestrian trajectory prediction.
  \item \textbf{High-angle view}: This is a view captured from a high vantage point, such as a camera mounted on a pole or building. High-angle view provides a wider field of view and captures the movement of vehicles or pedestrians in a larger area.
\end{itemize}

In deep learning trajectory prediction, the choice of POV can have a significant impact on the accuracy of the model, and often, multiple POV's are used in combination to improve prediction performance.


\subsection{Graph Isomorphism Networks}
A GIN is made up of several layers of graph convolutional operations, which are used to process the graph structure and update the features of the nodes. These operations are designed to be permutation-invariant, meaning they are able to handle graphs with different numbers of nodes and edges, and different node and edge labels. GINs can also use attention mechanisms to weight the importance of different nodes or edges in the graph, allowing the network to focus on the most relevant information for the task at hand.

One of the key features of GINs is that they use a multi-layer perceptron (MLP) as the readout function, which allows them to learn expressive representations of the graph structure. This readout function is applied to the node features after the final graph convolutional operation and is used to make predictions or perform classification. Additionally, GINs can be trained using the standard backpropagation algorithm and can be applied to various graph-based tasks such as node classification, link prediction, and graph classification. The main advantage of GINs is that they are able to effectively model the interactions between multiple entities in a graph, which is important for accurate predictions in graph-based tasks.

\subsection{Attention Mechanism}
Attention mechanisms are a type of neural network technique used to selectively focus on certain parts of the input data, allowing the network to better process and understand the information. They assist the network to focus on the most relevant information and make more accurate predictions. This allows the network to focus on the most relevant information and make more accurate predictions. In both CNN and GIN, attention mechanisms are often implemented as a module added to the network, which takes in the output of the previous layers and generates a set of attention weights. These attention weights are then used to weight the importance of different regions or nodes in the input data before passing it to the next layer.The main benefit of using attention mechanisms is that they allow the network to focus on the most relevant parts of the input data, which can improve the accuracy of the predictions.

Convolutional Block Attention Module (CBAM), is a type of attention mechanism that can be used to improve the performance of graph isomorphism networks. In a GIN, the goal is to determine whether two graphs are structurally identical. CBAM attention can be applied to this task by allowing the network to focus on specific regions or features of the input graphs. CBAM is made up of two parts: a channel-wise attention mechanism and a spatial attention mechanism.

The channel-wise attention mechanism is used to compute the importance of different feature channels in the input graphs. This is done by computing the average and standard deviation of the features across all spatial positions, and then using these statistics to weight the features. The spatial attention mechanism is used to compute the importance of different spatial positions within the input graphs. This is done by applying a convolutional operation to the input features, which generates a "heatmap" of attention weights for each position. By combining the channel-wise and spatial attention mechanisms, the CBAM attention allows the network to selectively focus on the most relevant regions and features of the input graphs, which can improve its ability to accurately classify graph isomorphism.


